CHCVerif: A Portfolio-Based Solver for Constrained Horn Clauses

Constrained Horn Clauses (CHCs) are widely adopted as intermediate representations for a variety of verification tasks, including safety checking, invariant synthesis, and interprocedural analysis. This paper introduces CHCVERIF, a portfolio-based CHC solver that adopts a software verification approach for solving CHCs. This approach enables us to reuse mature software verification tools to tackle CHC benchmarks, particularly those involving bitvectors and low-level semantics. Our evaluation shows that while the method enjoys only moderate success with linear integer arithmetic, it achieves modest success on bitvector benchmarks. Moreover, our results demonstrate the viability and potential of using software verification tools as backends for CHC solving, particularly when supported by a carefully constructed portfolio.

==> eptcsdata.tex <==
\providecommand{\firstpage}{40}
\providecommand{\publicationstatus}{Emanuele De Angelis, Florian Frohn (Eds.): 12th Workshop on\\
Horn Clauses for Verification and Synthesis (HCVS 2025)\\
EPTCS 434, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.434.6}{10.4204/EPTCS.434.6}}
\pdfoutput=1

